Extracting actionable information from microtexts

Microblogs such as Twitter represent a powerful source of information. Part of this information can be aggregated beyond the level of individual posts. Some of this aggregated information is referring to events that could or should be acted upon in the interest of e-governance, public safety, or other levels of public interest. Moreover, a significant amount of this information, if aggregated, could complement existing information networks in a non-trivial way. This dissertation proposes a semi-automatic method for extracting actionable information that serves this purpose. First, we show that predicting time to event is possible for both in-domain and cross-domain scenarios. Second, we suggest a method which facilitates the definition of relevance for an analyst's context and the use of this definition to analyze new data. Finally, we propose a method to integrate the machine learning based relevant information classification method with a rule-based information classification technique to classify microtexts. Fully automatizing microtext analysis has been our goal since the first day of this research project. Our efforts in this direction informed us about the extent this automation can be realized. We mostly first developed an automated approach, then we extended and improved it by integrating human intervention at various steps of the automated approach. Our experience confirms previous work that states that a well-designed human intervention or contribution in design, realization, or evaluation of an information system either improves its performance or enables its realization. As our studies and results directed us toward its necessity and value, we were inspired from previous studies in designing human involvement and customized our approaches to benefit from human input.

==> Chapters/Chapter1_sample.tex <==
\lhead{\emph{Introduction}}
\chapter{Introduction}

Twitter\footnote{\url{www.twitter.com}}, the social media platform, started in 2006 as a service to facilitate the sharing of personal updates with friends through SMS (Short Message Service). In accordance with the standard limit of 160 characters imposed on SMS messages, Twitter messages (`tweets') were bounded by a maximum of 140 characters, reserving 20 characters for a unique user address.\footnote{\url{http://www.140characters.com/2009/01/30/how-twitter-was-born/}} Twitter swiftly evolved into a medium through which users could `follow' one another and in which messages were open for anyone to read. While the user base and volume of tweets grew considerably over time, the 140 character limit to date remains effective. Information elements beyond the basic lexical content of messages offer alternative clues to interpret a Twitter post. For instance, the contents of a tweet could be understood by the {\em point in time} at which it was posted, which is stored as metadata in a post. In addition, the {\em hashtag} (`\#') surfaced as a convention to summarise the topic or emotion of a tweet. Not only are such contextual elements essential for communication through microblogs, they also make it possible to computationally model the relation between words in tweets and their context. An evident utility of such an effort is the automatic detection of real-world events and trending topics in the Twitter stream of messages, as well as a summary of related opinions and emotion. In this thesis, we study approaches to leverage temporal information and hashtags in tweets, in order to build a system that continuously generates overviews of public events, and that is sensitive to event aspects such as periodicity and emotion. 

The overarching aim of this thesis is to expose the popular experiences and feelings towards events that can be disclosed from a high volume of tweets. This aim accumulates in `\#anticipointment'. As a catchy portmanteau of anticipation and disappointment, the word `anticipointment' is used to either denote the positive expectation of a future event that is followed by a letdown\footnote{\url{http://nancyfriedman.typepad.com/away_with_words/2011/12/word-of-the-week-anticipointment.html}} or the anticipation of disappointment itself. As a platform through which experiences are abundantly anticipated and evaluated, Twitter might exhibit anticipointment frequently. The two approaches proposed in this thesis, aimed at detecting events and emotion, ultimately converge into the automatic detection of public anticipointment. The thesis title also points to the primary building blocks of our studies: hashtags and time. In the title, hashtags are reflected by the hashtag marker that precedes `anticipointment', and time is a necessary anchor for the concepts of anticipation and disappointment, as well as the transition between these emotions as part of anticipointment. 

This thesis is divided into three parts: `Time-based patterns', `Hashtag-based patterns', and `Expectations and retrospections on Twitter: Converging hashtags and time'. The first part comprises studies to infer the time interval between tweets and the start of an event, detect real-world events by leveraging either word frequencies over time or explicit time references in tweets, and identify periodic patterns from detected events. The second part explores the use of hashtags to model sarcasm and a variety of emotions. The last part combines the outcomes of the previous two sections into a computational analysis of the emotions before and after a diverse set of automatically detected events. 

The studies in this thesis have been conducted as part of the Information Retrieval for Information Services project (INFINITI) within the COMMIT/ research community.\footnote{\url{http://www.commit-nl.nl/projects/information-retrieval-for-information-services}}  All studies have been applied to Dutch tweets harvested within the TwiNL framework.\footnote{\url{http://www.ru.nl/lst/projects/twinl/}} Based on these studies, we assembled a system that processes Dutch tweets as they are posted. Its output is made available as the `Lama Events' Web application.\footnote{\url{http://applejack.science.ru.nl/lamaevents/}} 
%Although we have focused on the Dutch Twitterverse, the approaches that we study can to a large extent be transferred to any other language on Twitter. 

In the remainder of the introduction, we provide a motivation of the research (Section \ref{motivation}), describe the underlying research questions (Section \ref{rqs}) and give an outline of the thesis (Section \ref{outline}).

\section{Motivation} \label{motivation}

\subsection{Approach} \label{approach}

This thesis is set in the Artificial Intelligence tradition to build an intelligent entity \cite{Russell+95}, that in our case takes the form of an Information System. On the most basic level, Information Systems provide human end users with information of value in a given context. Such a system often has access to a voluminous database from which it distills information. The user itself is only presented with the output, and does not have to be proficient in the underlying software or hardware \cite{Wasserman80}. We develop software to find information from a stream of tweets, in the form of events and some of their aspects, and provide the user with a sensible overview of automatically detected events. 

In aiming to filter and transform the Twitter stream into useful information, our research connects to several fields. The first is the field of Time Series Analysis. As an area of Statistics, Time Series Analysis is a collection of methods that deal with observations made sequentially over time \cite{Chatfield13}. In this thesis, the field is predominantly reflected in our effort to highlight words that display `bursty' behaviour \cite{Kleinberg03}, and that thereby may signify real-world events. Second, our research relates to the field of Social Sensing, which aims to make sense of distributed observations about the world. By consulting tweets to detect real-world events, these sensors enable `social data scavenging', where the participants agree to the fact that their posts are in the public domain, while at the same time they are unaware of how their information is used \cite{Wang+15}. 
%Social Sensing primarily deals with assessing the reliability of observations. 
A third field that our research connects to lacks a common denominator, but can be formulated as `Mining the thought Web': the development of smart tools to interpret the millions of thoughts that are posted on Social Media platforms in real-time and connect them to subjects and events.\footnote{\url{http://techcrunch.com/2009/02/15/mining-the-thought-stream/}} Within this pursuit, our studies mostly relate to Sentiment Analysis, which encompasses the computational detection of opinion, sentiment, and subjectivity in text \cite{Pang+08}. In comparison to Social Sensing, the focus of this field is on thoughts and feelings rather than events in the real world. We aim at mining for both types of information. 

Despite its different fields of inspiration, the unifying characteristic of this thesis is that we lean heavily on `Collective Intelligence' or `The wisdom of the crowd'; the idea that a group as a whole knows more than any selection of experts \cite{Surowiecki05}. An estimated total of 303 million tweets were posted per day in January 2016\footnote{\url{http://uk.businessinsider.com/tweets-on-twitter-is-in-serious-decline-2016-2}} and an average of 732 thousand Dutch tweets could be crawled in the TwiNL framework per day in 2016.\footnote{It should be noted that this average was a lot higher up to the summer of 2014, but has since then been in decline (see for the exact numbers in the case of TwiNL \url{http://145.100.59.120/counts/} or navigate from \url{http://twiqs.nl})} Following the common practice on Twitter to share experiences and thoughts of personal importance, the collective of these posts arguably hosts a broad diversity of information about the world in real-time. We leverage collective intelligence to automatically detect the versatility and prominence of events and words to express emotions in Twitter. Essential elements in this pursuit are {\em contextual anchors}.

Contextual anchors can be defined as elements in a dataset that aggregate instances by a certain characteristic. Examples of anchors in Twitter are the geolocation that anchors tweets to their location, the user name that anchors tweets to their author, and the URL that relates tweets to information sources outside of Twitter. Anchors can be used to learn more about a target in a data-driven fashion. For example, by aggregating tweets that share a certain location from which they were posted, information about this location can be deduced from the remaining data in these tweets, such as the text. The contextual anchors that we use in this thesis are time and hashtags. 

Time is a useful anchor to detect events. While events can take many forms, we focus on events that take place within the limits of a single date. In accordance, tweets can be aggregated by their reference to the same date, and events can be identified as prominent words or phrases in these tweets. Effectively, these words or phrases might describe various types of events. We aim to detect events of any type, but do focus on significant events, e.g. events that might be reported in the news media \cite{McMinn+13} and that are hence of interest to a large group of people. %Such events are arguably of interest to most end users of the information system. 
We studied two approaches to link tweets to a date and thereby detect significant events. 

Hashtags are a potentially useful basis to model the language of emotions and rhetorical figures. Twitter users commonly deploy them to refer to a topic or event, to explicate the valence of a tweet (\#sarcasm) or to describe the emotion that they feel when writing a tweet. From a computational perspective, a hashtag can be leveraged to train a model of the words that link strongly to the underlying concept referred to by the hashtag.. The model can henceforth be used to detect the presence of the concept automatically in tweets that do not include the hashtag. Such an endeavour is valuable, given the proportion in which hashtags are deployed on Twitter. About a quarter of all tweets\footnote{Based on 27.7 million, predominantly Dutch, tweets, extracted from TwiNL (see Section \ref{twinl})} include a hashtag. A data set based on tweets with hashtags may offer predictive information that can be applied to tweets without a hashtag. As an alternative to labelling examples of a target manually or specify the type of words to focus on, this approach makes it possible to model with little effort any concept that is sufficiently clearly denoted with a hashtag. In case a hashtag denotes an emotion or rhetorical figure, the words that surround this hashtag ideally reflect the prototypical contexts in which the emotion or rhetorical figure can be expressed, as well as the degree to which any word is linked to it. 
%We assess for several hashtags if they are useful aggregators in this respect.   
%Hashtags might be suitable to model emotions, where 

While the framework of our studies is constituted by these data-driven approaches, knowledge-driven components are indispensable for their implementation. For example, in order to link tweets to a date and detect events, we formulate rules to specify the linguistic phrases that might refer to a date. In addition, the hashtags that we use to train an emotion or rhetorical figure are selected based on human knowledge. Hence, these studies manifest how knowledge-driven and data-driven components can best be combined in pursuit of information extraction.        

%The challenge that comes with these approaches is that they thrive with a large volume of tweets, and consequently can only be valued in the context of this large volume. We deliberately do not restrict the kind of events to detect or the words by which an emotion is detected, and let this implementation emerge from as many tweets as can be collected. In accordance, the approaches can not be tested on a controlled set of tweets; the human scale only comes in after output has been produced. As the output easily exceeds what can reasonably be processed by humans, only part of it can be manually assessed. We choose to use confidence rankings and evaluate the output up to a certain rank, which shows the performance at the highest confidence and as confidence decreases. In addition, we obtain a sense of recall (e.g.: comparison of the output to the targets that could have been detected) by checking for the retrieval of targets that can be located based on world knowledge.   

\subsection{Utility}

The approaches that we study are aimed at the extraction of a broad overview of events and their characteristics from tweets as they are posted. A system with a broad and open scope has a number of benefits. First, its output is of potential interest to several target groups. It can assist tourists who want to know about popular events in a specific location and time frame, as well as organisers of an event or product release who want to monitor the popularity of their event in time, possibly in relation to competitive events. Intelligence agencies may also be interested in a system that can timely foresee a social gathering of potential threat to public security. Although the output is not designed for any specific target group, the flexibility of the system makes it possible to easily post-process and tune the extracted patterns to the demands of any target group. 
%For example, additional emotions can easily be modeled, provided that they are sufficiently posted in the context of one or more hashtags. 

A second benefit is the possibility to compare events on various dimensions, such as the degree of popularity, the level of aggression, or disappointment, and rank them accordingly. The quantity and diversity of events allow for ranking and highlighting the most extreme cases, providing insights on a broad level. In the current thesis, this opportunity is explored in studies on periodicity detection and the detection of emotion in tweets that relate to a large number of events. 

Third, the system does not restrict the words that are used to refer to an event or express an emotion, and may thereby disclose output that is not found by any specialised system. In such specialised systems, the features to find a target are to a larger extent pre-specified. In contrast, our system makes no assumptions about the relative importance of input features and may discover strong predictors in features that we had not expected.
%The output from our system may help to refine the model of a specialised system. 

Finally, the information that is highlighted based on our data-driven approaches can be used to study the concept that they link to. For example, the use of sarcasm on Twitter can be studied after modelling the words that are used in the context of `\#sarcasm'. Such a procedure complements existing manual corpus studies of sarcasm, or verbal irony \cite{Burgers+11}.  

\subsection{Data} \label{twinl} 

Throughout this thesis we make use of the tweets that are collected within the TwiNL framework.\footnote{\url{http://www.ru.nl/lst/projects/twinl/}} These tweets are collected continuously from the Twitter API from December 2010 onward on the basis of a seed list of Dutch words and a dynamic list of the most active Dutch Twitter users \cite{TjongKimSang+13}. The harvesting is limited; TwiNL harvests an estimated half of all Dutch tweets. Nonetheless, the benefit of TwiNL is that it keeps a record of tweet IDs since December 2010, while the Twitter search API currently only returns tweets that were posted in the most recent seven days.\footnote{\url{https://dev.twitter.com/rest/public/search}} The long span of tweets in TwiNL enables us to research periodic event patterns and makes it possible to collect many tweets by querying for certain hashtags. For example, querying TwiNL for tweets that mention \#not in a window spanning December 2010 until January 2013 yields 353,758 tweets, and a search for tweets with \#zinin (`looking forward to it') between December 2010 and October 2015 results in 606,310 tweets.    

The use of Twitter data has two important implications. The first is that it might be tempting, based on the high number of tweets that are posted, to relate the patterns that are found in Twitter to the society as a whole. Studies have shown that the demographics of Twitter users do not reflect the demographics of a society \cite{Mislove+11}. The high number of posts do allow, however, for relatively accurate measurements of public opinion and approximate, for example, the outcomes of an election \cite{Sang+11,Digrazia+13,Sanders+13}, but this should not be seen as a consistent quality \cite{Gayo12}. 
%For this reason, we do not generalise the patterns that we see in Twitter in any way to a context outside of the confines of this platform. 

Second, Twitter is a volatile data source. The Twitter terms of service \footnote{\url{https://twitter.com/tos?lang=en}} state that users by default agree to post their messages in the public domain, which means that tweets can be read by anyone and harvested by third parties, as far as Twitter chooses to share its data. Users are allowed to remove tweets or make their account private, after which their tweets are invisible for any party outside their follower circle. Researchers are allowed to keep a database of tweets that they harvested, but cannot share tweets with other researchers. However, the unique IDs of tweets can be shared, based on which the content of the tweets can be queried from the Twitter API. Any tweet that has been removed or screened will not be returned from the API, which means that any research that is conducted based on Twitter posts can not be reproduced with the original dataset. In a study into indicators of tweet deletion, \citeauthor{Petrovic+13} experimented with a data set of 75 million tweets, of which 2.4 million tweets (3.2\%) were deleted within a month time. For this reason, our research is aimed at developing a system that processes tweets in real-time. The outcomes of our evaluations are meant to be descriptive of such a context. We do share tweet IDs of every study, as well as the information that has been extracted from them.\footnote{In each section that discusses a dataset in this thesis, we point to the URL at which we have placed the related tweet IDs}   

\section{Research Questions} \label{rqs}

The main problem statement that drives the studies in this thesis is the following: \\

\begin{adjustwidth}{1cm}{}
\textbf{PS: How can we discover time-anchored events and their characteristics from a stream of Twitter messages?} \\
\end{adjustwidth}

As motivated in Section \ref{approach}, the events that we target typically take place on a single day, and are thereby anchored in time. Research questions 1 and 2 address the detection of such events from Twitter. The remaining research questions drive the work to analyse event characteristics. An introduction of all research questions, as well as an overview of the contributions of our work, is given below. 

The date at which future events take place might be shared in tweets that refer to it. Extracting this information is especially useful to learn about events that are not known to the general public, such as a demonstration or local party. Obviously, it is most useful to extract such information as early as possible. In a stream of tweets that refer to an event, by means of a common hashtag or event phrase, only part of the references to future dates might relate to the event itself. The objective is then to find the most optimal approach to extract the event date, in terms of speed and accuracy: \\


%Given event describing hashtags or phrases, tweets that refer to the same event could be aggregated. It is not known, however  terms can be used to aggregate tweets that refer 
%Messages on Twitter are said to most quickly report on events as they occur. Likewise,  In line with this intuition, we study the information about the date of an event that is contained in tweets that anticipate the event. By collecting tweets that refer to a known event with a distinctive hashtag, we can isolate such an `event stream'. Concretely, we categorise the tweets by their temporal distance to the event date and study the relation between this distance and the text in tweets. The underlying research question is as follows: \\

\begin{adjustwidth}{1cm}{}
\textbf{RQ 1: Given a stream of tweets that refer to the same event, how accurately and early can we infer the number of days until the start of this event?} \\
\end{adjustwidth}

%\begin{figure}[t]
%  \centering
%  \includegraphics[scale=0.4]{Figures/referendum_plot1.pdf}\label{bu}
%  \caption{The number of tweets per day that mention `referendum' and `referendum' in combination with a reference to the future date of April 6, 2016, depicted in the scale of the former}
%  \label{time_plot1}
%\end{figure}

%\begin{figure}[t]
%  \centering
%  \includegraphics[scale=0.4]{Figures/referendum_plot2.pdf}\label{tr} 
%  \caption{The number of tweets per day that mention `referendum' and `referendum' in combination with a reference to the future date of April 6, 2016, depicted in the scale of the latter}
%  \label{time_plot2}
%\end{figure}

While a known event can be leveraged to obtain insights into temporal information in tweets, this temporal information can in turn be deployed as starting point to detect events. We compare two approaches to using temporal information for event detection. The first is to observe the time when tweets are posted. The second is to focus on the temporal information that might be given in the text of a tweet. To illustrate the two approaches, we plotted in Figure \ref{time_plot1} the frequency of tweets that refer to a referendum held in the Netherlands on April 6, 2016, either by just mentioning the word `referendum' or by mentioning the word `referendum' along with a future reference to the date of this event. The plots are depicted in the scale of all tweets with this term. The date of the event can clearly be recognised as the point where the number of tweets is magnitudes higher than the frequency at any other point. This reflects that Twitter users are mostly inclined to tweet about an event as it occurs. Following this behaviour, events can be detected by counting words that are mentioned on Twitter over time, and highlighting words that show a sudden increase. This word frequency that might indicate an event coincides with the time at which the event takes place. We refer to event detection based on this direct indication as `burstiness-based event detection'.

The line in Figure \ref{time_plot1} that describes the number of tweets with a textual reference to the event date is barely visible, as it stays close to the horizontal axis. As a comparison, we depicted the same plots in the scale of this line in Figure \ref{time_plot2}. The frequency of all tweets is partly visible in this plot, before shooting through the roof about seven weeks before the event. The number of tweets that refer to the date of the event are more scattered over time and only show a subtle increase as the event approaches, with a small peak close to the event. Rather than showing a pattern by their time stamp, it is the content of these tweets that reveals a dominant event date. This signal can be leveraged by scanning tweets for the presence of a time expression, following the study linked to RQ1, and subsequently finding words that potentially describe an event in the remainder of these tweets. We refer to this more indirect approach to event detection as `time reference-based event detection'.

%A second variant of temporal information is the display of textual markers in tweets. Based on RQ1 we develop methods for the detection of textual markers that are most indicative of the time-to-event of a set of tweets. A selection of these markers can subsequently be used as possible indicators of an event date. The words that describe this potential event could then be found in the remainder of the words in tweets. This is a more indirect type of temporal information for event detection. The textual references in tweets to the date of an event might be , but can be linked by referencing a similar future date and similar terms. We refer to this type of event detection as `time reference-based event detection'.

The development of both burstiness-based and time reference-based event detection systems is driven by the following two research questions: \\
%We will apply both burstiness-based and time reference-based event detection, which connects to the following research questions: \\

\begin{adjustwidth}{1cm}{}
\textbf{RQ 2a: To what extent can events be detected from Twitter by means of burstiness-based event detection?} \\
\textbf{RQ 2b: To what extent can events be detected from Twitter by means of time reference-based event detection?} \\
\end{adjustwidth}

Based on the effort to automatically detect events as part of RQ 2, we can subsequently apply event detection to the long span of tweets that is available in the TwiNL framework. The resulting set of events makes it possible to zoom out and move the attention from temporal information in tweets to temporal information in events. One follow-up task is to identify events that recur periodically, so that we can predict their next recurrence even without following the Twitter stream. We compare two approaches to identify periodic events in a bottom-up fashion. The first is based on the intervals in days between occurrences of similarly described events. The second is driven by calendar information. We ask the following research question: \\

\begin{adjustwidth}{1cm}{}
\textbf{RQ 3: Given a set of detected events from Twitter over an extended period of time, to what extent can periodic events be identified?} \\
\end{adjustwidth}

Shifting our focus from time to hashtags as anchor within the Twitter stream, we performed experiments to test the usefulness of hashtags in modelling the language of sarcasm and emotions. Although emotions have a more overt relation to events than sarcasm, sarcasm detection can potentially be used as a filter for sentiment detection. 
%that can potentially benefit from the many tweets that are denoted with a sarcasm-related hashtag.
 We argue that the usefulness of a hashtag depends on two factors. The first is whether a hashtag is deployed in a consistent way by Twitter users. For example, the hashtag `\#funny' might denote a joke or a strange situation, or be used in a sarcastic way. A high ambiguity makes it difficult to learn the context of a hashtag, and renders the automatically learned detector useless. The second factor is whether the hashtag reflects the emotion that is present in the rest of the words, or whether it adds the concept to the message that in itself does not express the emotion. To illustrate, consider the example tweets below.

\begin{enumerate}
    \item Doing homework \#boring
    \item I would rather do something else, but unfortunately I have to do my homework \#boring 
\end{enumerate}

In the first example, the phrase `doing homework' does not convey the lack of excitement of the author about this activity. The boredom is purely reflected in the hashtag. In contrast, the textual part of the second example clearly conveys a certain boredom about the prospect of doing homework, which is only repeated or strengthened by the hashtag. In order to train a model of the emotion of boredom, usage of the hashtag as in the second example is obviously preferable over the first. As it is not clear beforehand %to what extent the two factors apply to a hashtag that conveys an emotion or sarcasm, and by extension 
how useful any hashtag is as training label, we empirically test the usefulness for several hashtags. This is related to the research question below: \\

\begin{adjustwidth}{1cm}{}
\textbf{RQ 4: To what extent can figurative speech or emotion in tweets be detected based on hashtag-annotations?} \\
\end{adjustwidth}

We can combine the insights gained from answering RQ 2 and RQ 4 to detect the emotion in tweets that relate to automatically detected events. One application of such a combination is the detection of emotions that relate to expectations and actual experience. We set out to study occurrences of anticipointment by automatically detecting the emotion of positive expectation in tweets before events, and disappointment in tweets after events. By also including satisfaction, we can research whether a correlation exists between these three emotions: \\

\begin{adjustwidth}{1cm}{}
\textbf{RQ 5: What is the strength of the correlation between the collective expression of positive expectation before events and disappointment and satisfaction after events on Twitter?} \\
\end{adjustwidth}

\section{Thesis contributions}

This thesis aims for a number of contributions to the fields mentioned above. First, it presents three new tasks: identifying the number of days until an event starts from a stream of event tweets, detecting periodicity from Twitter events and comparing the emotion before and after events as expressed on Twitter. Second, it provides further insights on the widely studied tasks of event detection, sarcasm detection and emotion detection. Third, all studies in this thesis give insight into system performance in a realistic setting of streaming Twitter posts, where the output is automatically ranked in order to select output for manual evaluation. Fourth, the components that were developed and tested in the separate studies are assembled into the Lama Events Web application\footnote{\url{http://applejack.science.ru.nl/lamaevents/}} that processes tweets in real-time.

%\begin{enumerate}^
	%\item The first study on 
	%\item The further development of existing work on event detection, sarcasm detection and emotion detection.
    	%\item The first research on 
    	%\item The first research on the comparison of emotion before and after events as expressed on Twitter
    %	\item Evaluation of these tasks in a realistic setting of streaming Twitter posts
%	\item The assembly of several applications into a demo system that processes streaming tweets. 
%\end{enumerate} 

\section{Thesis outline} \label{outline}

Part \ref{part1} comprises studies on time-based patterns. In Chapter 2 we start working with hashtags that are strongly linked to known football events, in order to examine the Twitter text that surrounds such a hashtag for information on the event date. Using both time features and word $n$-gram features, we compare the performance of a rule-based system and machine learning on accurately estimating the time-to-event at any point in a stream of hashtag-aggregated event tweets. We subsequently evaluate performance on a set of open-domain events. In Chapter 3, we start from two months in the total Twitter stream of TwiNL and set out to identify hashtags and event phrases that signify an event, based on the sudden rise in frequency of such tokens. In Chapter 4, we pursue the same goal, but identify events as the induced date of forward referring time expressions that link strongly to a certain word or phrase. In Chapter 5, we set out to identify periodic events by applying event detection on a span of over four years and looking for periodic intervals or calendar patterns related to similar event terms.

Part \ref{part2} features research on hashtag-based patterns. In Chapter 6, we select a combination of hashtags that might be deployed by Twitter users as a marker of sarcasm that flips the polarity of their message. We test the effectiveness of these hashtags as training label for machine learning on a total day of Twitter messages, and analyse the characteristics of sarcasm in tweets. In Chapter 7, we extend the procedure of Chapter 6 to a total of 24 hashtags that link to several course-grained fine-grained emotions, and assess the usefulness of these hashtags as annotation label for emotion detection. 

In Part \ref{part3}, we combine the lines of research in Part \ref{part1} and Part \ref{part2} in a study of the emotions before and after a wide range of events. We train a classifier to recognise positive expectation, disappointment and satisfaction, and apply it to a large number of pre-event and post-event tweets. For each of the emotions, an aggregate emotion score is derived for each event based on the tweet classifications. We make use of this aggregate score to calculate the correlation between any of the three emotions, highlight the events that manifest the most extreme patterns, and analyse the emotion for a sequence of known events.


==> Chapters/SIKSDissertations.tex <==

\chapter*{\Huge SIKS Dissertation Series}

\scriptsize
\setlist[enumerate]{topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex}

%\begin{longtable}{@{}l@{ }l@{\hspace{1em}}X}
\begin{longtabu}{@{}l@{ }l@{\hspace{1em}}X}
\toprule
1998	&	 01	&	 Johan van den Akker (CWI), DEGAS - An Active, Temporal Database of Autonomous Objects \\
	&	 02	&	 Floris Wiesman (UM), Information Retrieval by Graphically Browsing Meta-Information \\
	&	 03	&	 Ans Steuten (TUD), A Contribution to the Linguistic Analysis of Business Conversations within the Language/Action Perspective \\
	&	 04	&	 Dennis Breuker (UM), Memory versus Search in Games \\
	&	 05	&	 E.W.Oskamp (RUL), Computerondersteuning bij Straftoemeting \\
\midrule
1999	&	 01	&	 Mark Sloof (VU), Physiology of Quality Change Modelling; Automated modelling of Quality Change of Agricultural Products \\
	&	 02	&	 Rob Potharst (EUR), Classification using decision trees and neural nets \\
	&	 03	&	 Don Beal (UM), The Nature of Minimax Search \\
	&	 04	&	 Jacques Penders (UM), The practical Art of Moving Physical Objects \\
	&	 05	&	 Aldo de Moor (KUB), Empowering Communities: A Method for the Legitimate User-Driven Specification of Network Information Systems \\
	&	 06	&	 Niek J.E. Wijngaards (VU), Re-design of compositional systems \\
	&	 07	&	 David Spelt (UT), Verification support for object database design \\
	&	 08	&	 Jacques H.J. Lenting (UM), Informed Gambling: Conception and Analysis of a Multi-Agent Mechanism
	for Discrete Reallocation. \\
\midrule
2000	&	 01	&	 Frank Niessink (VU), Perspectives on Improving Software Maintenance \\
	&	 02	&	 Koen Holtman (TUE), Prototyping of CMS Storage Management \\
	&	 03	&	 Carolien M.T. Metselaar (UVA), Sociaal-organisatorische gevolgen van kennistechnologie; een procesbenadering en actorperspectief. \\
	&	 04	&	 Geert de Haan (VU), ETAG, A Formal Model of Competence Knowledge for User Interface Design \\
	&	 05	&	 Ruud van der Pol (UM), Knowledge-based Query Formulation in Information Retrieval. \\
	&	 06	&	 Rogier van Eijk (UU), Programming Languages for Agent Communication \\
	&	 07	&	 Niels Peek (UU), Decision-theoretic Planning of Clinical Patient Management \\
	&	 08	&	 Veerle Coup (EUR), Sensitivity Analyis of Decision-Theoretic Networks \\
	&	 09	&	 Florian Waas (CWI), Principles of Probabilistic Query Optimization \\
	&	 10	&	 Niels Nes (CWI), Image Database Management System Design Considerations, Algorithms and Architecture \\
	&	 11	&	 Jonas Karlsson (CWI), Scalable Distributed Data Structures for Database Management \\
\midrule
2001	&	 01	&	 Silja Renooij (UU), Qualitative Approaches to Quantifying Probabilistic Networks \\	
	&	 02	&	 Koen Hindriks (UU), Agent Programming Languages: Programming with Mental Models \\
	&	 03	&	 Maarten van Someren (UvA), Learning as problem solving \\
	&	 04	&	 Evgueni Smirnov (UM), Conjunctive and Disjunctive Version Spaces with Instance-Based Boundary Sets \\
	&	 05	&	 Jacco van Ossenbruggen (VU), Processing Structured Hypermedia: A Matter of Style \\
	&	 06	&	 Martijn van Welie (VU), Task-based User Interface Design \\
	&	 07	&	 Bastiaan Schonhage (VU), Diva: Architectural Perspectives on Information Visualization \\
	&	 08	&	 Pascal van Eck (VU), A Compositional Semantic Structure for Multi-Agent Systems Dynamics. \\
	&	 09	&	 Pieter Jan 't Hoen (RUL), Towards Distributed Development of Large Object-Oriented Models Views of Packages as Classes \\
	&	 10	&	 Maarten Sierhuis (UvA), Modeling and Simulating Work Practice BRAHMS: a multiagent modeling and simulation language for work practice analysis and design \\
	&	 11	&	 Tom M. van Engers (VUA) Knowledge Management: The Role of Mental Models in Business Systems Design \\

\midrule
2002-01 Nico Lassing (VU), Architecture-Level Modifiability Analysis \ 2002-02 Roelof van Zwol (UT)
Modelling and searching web-based document collections
        
2002-03 Henk Ernst Blok (UT)
        Database Optimization Aspects for Information Retrieval \ 2002-04 Juan Roberto Castelo Valdueza (UU)
      	The Discrete Acyclic Digraph Markov Model in Data Mining
      
2002-05 Radu Serban (VU)
      	The Private Cyberspace Modeling Electronic, Environments inhabited by Privacy-concerned Agents \ 2002-06 Laurens Mommers (UL)
      	Applied legal epistemology; Building a knowledge-based ontology of
      	the legal domain 
              
2002-07 Peter Boncz (CWI)
      	Monet: A Next-Generation DBMS Kernel For Query-Intensive
      	Applications
              
2002-08 Jaap Gordijn (VU)
      	Value Based Requirements Engineering: Exploring Innovative
      	E-Commerce Ideas \ 2002-09 Willem-Jan van den Heuvel(KUB)
       	Integrating Modern Business Applications with Objectified Legacy
       	Systems 
      
2002-10 Brian Sheppard (UM) , Towards Perfect Play of Scrabble 
      
2002-11	Wouter C.A. Wijngaards (VU), Agent Based Modelling of Dynamics: Biological and Organisational Applications \ 2002-12	Albrecht Schmidt (Uva), Processing XML in Database Systems \ 2002-13	Hongjing Wu (TUE), A Reference Architecture for Adaptive Hypermedia Applications \ 2002-14 Wieke de Vries (UU), Agent Interaction: Abstract Approaches to Modelling, Programming and Verifying Multi-Agent Systems \ 2002-15	Rik Eshuis (UT), Semantics and Verification of UML Activity Diagrams for Workflow Modelling \ 2002-16	Pieter van Langen (VU), The Anatomy of Design: Foundations, Models and Applications \ 2002-17	Stefan Manegold (UVA), Understanding, Modeling, and Improving Main-Memory Database Performance \
\midrule
2011	&	 01	&	 Botond Cseke (RUN), Variational Algorithms for Bayesian Inference in Latent Gaussian Models\\
	&	 02	&	 Nick Tinnemeier (UU), Organizing Agent Organizations. Syntax and Operational Semantics of an Organization-Oriented Programming Language\\
	&	 03	&	 Jan Martijn van der Werf (TUE), Compositional Design and Verification of Component-Based Information Systems\\
	&	 04	&	 Hado van Hasselt (UU), Insights in Reinforcement Learning; Formal analysis and empirical evaluation of temporal-difference\\
	&	 05	&	 Bas van der Raadt (VU), Enterprise Architecture Coming of Age - Increasing the Performance of an Emerging Discipline.\\
	&	 06	&	 Yiwen Wang (TUE), Semantically-Enhanced Recommendations in Cultural Heritage\\
	&	 07	&	 Yujia Cao (UT), Multimodal Information Presentation for High Load Human Computer Interaction\\
	&	 08	&	 Nieske Vergunst (UU), BDI-based Generation of Robust Task-Oriented Dialogues\\
	&	 09	&	 Tim de Jong (OU), Contextualised Mobile Media for Learning\\
	&	 10	&	 Bart Bogaert (UvT), Cloud Content Contention\\
	&	 11	&	 Dhaval Vyas (UT), Designing for Awareness: An Experience-focused HCI Perspective\\
	&	 12	&	 Carmen Bratosin (TUE), Grid Architecture for Distributed Process Mining\\
	&	 13	&	 Xiaoyu Mao (UvT), Airport under Control. Multiagent Scheduling for Airport Ground Handling\\
	&	 14	&	 Milan Lovric (EUR), Behavioral Finance and Agent-Based Artificial Markets\\
	&	 15	&	 Marijn Koolen (UvA), The Meaning of Structure: the Value of Link Evidence for Information Retrieval\\
	&	 16	&	 Maarten Schadd (UM), Selective Search in Games of Different Complexity\\
	&	 17	&	 Jiyin He (UVA), Exploring Topic Structure: Coherence, Diversity and Relatedness\\
	&	 18	&	 Mark Ponsen (UM), Strategic Decision-Making in complex games\\
	&	 19	&	 Ellen Rusman (OU), The Mind's Eye on Personal Profiles\\
	&	 20	&	 Qing Gu (VU), Guiding service-oriented software engineering - A view-based approach\\
	&	 21	&	 Linda Terlouw (TUD), Modularization and Specification of Service-Oriented Systems\\
	&	 22	&	 Junte Zhang (UVA), System Evaluation of Archival Description and Access\\
	&	 23	&	 Wouter Weerkamp (UVA), Finding People and their Utterances in Social Media\\
	&	 24	&	 Herwin van Welbergen (UT), Behavior Generation for Interpersonal Coordination with Virtual Humans On Specifying, Scheduling and Realizing Multimodal Virtual Human Behavior\\
	&	 25	&	 Syed Waqar ul Qounain Jaffry (VU), Analysis and Validation of Models for Trust Dynamics\\
	&	 26	&	 Matthijs Aart Pontier (VU), Virtual Agents for Human Communication - Emotion Regulation and Involvement-Distance Trade-Offs in Embodied Conversational Agents and Robots\\
	&	 27	&	 Aniel Bhulai (VU), Dynamic website optimization through autonomous management of design patterns\\
	&	 28	&	 Rianne Kaptein (UVA), Effective Focused Retrieval by Exploiting Query Context and Document Structure\\
	&	 29	&	 Faisal Kamiran (TUE), Discrimination-aware Classification\\
	&	 30	&	 Egon van den Broek (UT), Affective Signal Processing (ASP): Unraveling the mystery of emotions\\
	&	 31	&	 Ludo Waltman (EUR), Computational and Game-Theoretic Approaches for Modeling Bounded Rationality\\
	&	 32	&	 Nees-Jan van Eck (EUR), Methodological Advances in Bibliometric Mapping of Science\\
	&	 33	&	 Tom van der Weide (UU), Arguing to Motivate Decisions\\
	&	 34	&	 Paolo Turrini (UU), Strategic Reasoning in Interdependence: Logical and Game-theoretical Investigations\\
	&	 35	&	 Maaike Harbers (UU), Explaining Agent Behavior in Virtual Training\\
	&	 36	&	 Erik van der Spek (UU), Experiments in serious game design: a cognitive approach\\
	&	 37	&	 Adriana Burlutiu (RUN), Machine Learning for Pairwise Data, Applications for Preference Learning and Supervised Network Inference\\
	&	 38	&	 Nyree Lemmens (UM), Bee-inspired Distributed Optimization\\
	&	 39	&	 Joost Westra (UU), Organizing Adaptation using Agents in Serious Games\\
	&	 40	&	 Viktor Clerc (VU), Architectural Knowledge Management in Global Software Development\\
	&	 41	&	 Luan Ibraimi (UT), Cryptographically Enforced Distributed Data Access Control\\
	&	 42	&	 Michal Sindlar (UU), Explaining Behavior through Mental State Attribution\\
	&	 43	&	 Henk van der Schuur (UU), Process Improvement through Software Operation Knowledge\\
	&	 44	&	 Boris Reuderink (UT), Robust Brain-Computer Interfaces\\
	&	 45	&	 Herman Stehouwer (UvT), Statistical Language Models for Alternative Sequence Selection\\
	&	 46	&	 Beibei Hu (TUD), Towards Contextualized Information Delivery: A Rule-based Architecture for the Domain of Mobile Police Work\\
	&	 47	&	 Azizi Bin Ab Aziz (VU), Exploring Computational Models for Intelligent Support of Persons with Depression\\
	&	 48	&	 Mark Ter Maat (UT), Response Selection and Turn-taking for a Sensitive Artificial Listening Agent\\
	&	 49	&	 Andreea Niculescu (UT), Conversational interfaces for task-oriented spoken dialogues: design aspects influencing interaction quality\\
	
\midrule
2012&	 01	&	 Terry Kakeeto (UvT), Relationship Marketing for SMEs in Uganda\\
	&	 02	&	 Muhammad Umair (VU), Adaptivity, emotion, and Rationality in Human and Ambient Agent Models\\
	&	 03	&	 Adam Vanya (VU), Supporting Architecture Evolution by Mining Software Repositories\\
	&	 04	&	 Jurriaan Souer (UU), Development of Content Management System-based Web Applications\\
	&	 05	&	 Marijn Plomp (UU), Maturing Interorganisational Information Systems\\
	&	 06	&	 Wolfgang Reinhardt (OU), Awareness Support for Knowledge Workers in Research Networks\\
	&	 07	&	 Rianne van Lambalgen (VU), When the Going Gets Tough: Exploring Agent-based Models of Human Performance under Demanding Conditions\\
	&	 08	&	 Gerben de Vries (UVA), Kernel Methods for Vessel Trajectories\\
	&	 09	&	 Ricardo Neisse (UT), Trust and Privacy Management Support for Context-Aware Service Platforms\\
	&	 10	&	 David Smits (TUE), Towards a Generic Distributed Adaptive Hypermedia Environment\\
	&	 11	&	 J.C.B. Rantham Prabhakara (TUE), Process Mining in the Large: Preprocessing, Discovery, and Diagnostics\\
	&	 12	&	 Kees van der Sluijs (TUE), Model Driven Design and Data Integration in Semantic Web Information Systems\\
	&	 13	&	 Suleman Shahid (UvT), Fun and Face: Exploring non-verbal expressions of emotion during playful interactions\\
	&	 14	&	 Evgeny Knutov (TUE), Generic Adaptation Framework for Unifying Adaptive Web-based Systems\\
	&	 15	&	 Natalie van der Wal (VU), Social Agents. Agent-Based Modelling of Integrated Internal and Social Dynamics of Cognitive and Affective Processes.\\
	&	 16	&	 Fiemke Both (VU), Helping people by understanding them - Ambient Agents supporting task execution and depression treatment\\
	&	 17	&	 Amal Elgammal (UvT), Towards a Comprehensive Framework for Business Process Compliance\\
	&	 18	&	 Eltjo Poort (VU), 	Improving Solution Architecting Practices\\
	&	 19	&	 Helen Schonenberg (TUE), What's Next? Operational Support for Business Process Execution\\
	&	 20	&	 Ali Bahramisharif (RUN), Covert Visual Spatial Attention, a Robust Paradigm for Brain-Computer Interfacing\\
	&	 21	&	 Roberto Cornacchia (TUD), Querying Sparse Matrices for Information Retrieval\\
	&	 22	&	 Thijs Vis (UvT), Intelligence, politie en veiligheidsdienst: verenigbare grootheden?\\
	&	 23	&	 Christian Muehl (UT), Toward Affective Brain-Computer Interfaces: Exploring the Neurophysiology of Affect during Human Media Interaction\\
	&	 24	&	 Laurens van der Werff (UT), Evaluation of Noisy Transcripts for Spoken Document Retrieval\\
	&	 25	&	 Silja Eckartz (UT), Managing the Business Case Development in Inter-Organizational IT Projects: A Methodology and its Application\\
	&	 26	&	 Emile de Maat (UVA), Making Sense of Legal Text\\
	&	 27	&	 Hayrettin Gurkok (UT), Mind the Sheep! User Experience Evaluation \& Brain-Computer Interface Games\\
	&	 28	&	 Nancy Pascall (UvT), Engendering Technology Empowering Women\\
	&	 29	&	 Almer Tigelaar (UT), Peer-to-Peer Information Retrieval\\
	&	 30	&	 Alina Pommeranz (TUD), Designing Human-Centered Systems for Reflective Decision Making\\
	&	 31	&	 Emily Bagarukayo (RUN), A Learning by Construction Approach for Higher Order Cognitive Skills Improvement, Building Capacity and Infrastructure\\
	&	 32	&	 Wietske Visser (TUD), 	Qualitative multi-criteria preference representation and reasoning\\
	&	 33	&	 Rory Sie (OUN), Coalitions in Cooperation Networks (COCOON)\\
	&	 34	&	 Pavol Jancura (RUN), Evolutionary analysis in PPI networks and applications\\
	&	 35	&	 Evert Haasdijk (VU), Never Too Old To Learn -- On-line Evolution of Controllers in Swarm- and Modular Robotics\\
	&	 36	&	 Denis Ssebugwawo (RUN), Analysis and Evaluation of Collaborative Modeling Processes\\
	&	 37	&	 Agnes Nakakawa (RUN), A Collaboration Process for Enterprise Architecture Creation\\
	&	 38	&	 Selmar Smit (VU), Parameter Tuning and Scientific Testing in Evolutionary Algorithms\\
	&	 39	&	 Hassan Fatemi (UT), Risk-aware design of value and coordination networks\\
	&	 40	&	 Agus Gunawan (UvT), Information Access for SMEs in Indonesia\\
	&	 41	&	 Sebastian Kelle (OU), Game Design Patterns for Learning\\
	&	 42	&	 Dominique Verpoorten (OU), Reflection Amplifiers in self-regulated Learning\\
	&	 43	&	 Withdrawn \\
	&	 44	&	 Anna Tordai (VU), On Combining Alignment Techniques\\
	&	 45	&	 Benedikt Kratz (UvT), A Model and Language for Business-aware Transactions\\
	&	 46	&	 Simon Carter (UVA), Exploration and Exploitation of Multilingual Data for Statistical Machine Translation\\
	&	 47	&	 Manos Tsagkias (UVA), Mining Social Media: Tracking Content and Predicting Behavior\\
	&	 48	&	 Jorn Bakker (TUE), Handling Abrupt Changes in Evolving Time-series Data\\
	&	 49	&	 Michael Kaisers (UM), Learning against Learning - Evolutionary dynamics of reinforcement learning algorithms in strategic interactions\\
	&	 50	&	 Steven van Kervel (TUD), Ontologogy driven Enterprise Information Systems Engineering\\
	&	 51	&	 Jeroen de Jong (TUD), Heuristics in Dynamic Sceduling; a practical framework with a case study in elevator dispatching\\
	
\midrule
2013&    01	&    Viorel Milea (EUR), News Analytics for Financial Decision Support\\
	&	 02	&	 Erietta Liarou (CWI), MonetDB/DataCell: Leveraging the Column-store Database Technology for Efficient and Scalable Stream Processing\\
	&	 03	&	 Szymon Klarman (VU), Reasoning with Contexts in Description Logics\\
	&	 04	&	 Chetan Yadati (TUD), Coordinating autonomous planning and scheduling\\
	&	 05	&	 Dulce Pumareja (UT), Groupware Requirements Evolutions Patterns\\
	&	 06	&	 Romulo Goncalves (CWI), The Data Cyclotron: Juggling Data and Queries for a Data Warehouse Audience\\
	&	 07	&	 Giel van Lankveld (UvT), Quantifying Individual Player Differences\\
	&	 08	&	 Robbert-Jan Merk (VU), Making enemies: cognitive modeling for opponent agents in fighter pilot simulators\\
	&	 09	&	 Fabio Gori (RUN), Metagenomic Data Analysis: Computational Methods and Applications\\
	&	 10	&	 Jeewanie Jayasinghe Arachchige (UvT), A Unified Modeling Framework for Service Design.\\
	&	 11	&	 Evangelos Pournaras (TUD), Multi-level Reconfigurable Self-organization in Overlay Services\\
	&	 12	&	 Marian Razavian (VU), Knowledge-driven Migration to Services\\
	&	 13	&	 Mohammad Safiri (UT), Service Tailoring: User-centric creation of integrated IT-based homecare services to support independent living of elderly\\
	&	 14	&	 Jafar Tanha (UVA), Ensemble Approaches to Semi-Supervised Learning Learning\\
	&	 15	&	 Daniel Hennes (UM), Multiagent Learning - Dynamic Games and Applications\\
	&	 16	&	 Eric Kok (UU), Exploring the practical benefits of argumentation in multi-agent deliberation\\
	&	 17	&	 Koen Kok (VU), The PowerMatcher: Smart Coordination for the Smart Electricity Grid\\
	&	 18	&	 Jeroen Janssens (UvT), Outlier Selection and One-Class Classification\\
	&	 19	&	 Renze Steenhuizen (TUD), Coordinated Multi-Agent Planning and Scheduling\\
	&	 20	&	 Katja Hofmann (UvA), Fast and Reliable Online Learning to Rank for Information Retrieval\\
	&	 21	&	 Sander Wubben (UvT), Text-to-text generation by monolingual machine translation\\
	&	 22	&	 Tom Claassen (RUN), Causal Discovery and Logic\\
	&	 23	&	 Patricio de Alencar Silva (UvT), Value Activity Monitoring\\
	&	 24	&	 Haitham Bou Ammar (UM), 	Automated Transfer in Reinforcement Learning\\
	&	 25	&	 Agnieszka Anna Latoszek-Berendsen (UM), 	Intention-based Decision Support. A new way of representing and implementing clinical guidelines in a Decision Support System\\
	&	 26	&	 Alireza Zarghami (UT), 	Architectural Support for Dynamic Homecare Service Provisioning\\
	&	 27	&	 Mohammad Huq (UT), 	Inference-based Framework Managing Data Provenance\\
	&	 28	&	 Frans van der Sluis (UT), 	When Complexity becomes Interesting: An Inquiry into the Information eXperience\\
	&	 29	&	 Iwan de Kok (UT), 	Listening Heads\\
	&	 30	&	 Joyce Nakatumba (TUE), 	Resource-Aware Business Process Management: Analysis and Support\\
	&	 31	&	 Dinh Khoa Nguyen (UvT), 	Blueprint Model and Language for Engineering Cloud Applications\\
	&	 32	&	 Kamakshi Rajagopal (OUN), 	Networking For Learning; The role of Networking in a Lifelong Learner's Professional Development\\
	&	 33	&	 Qi Gao (TUD), User Modeling and Personalization in the Microblogging Sphere\\
	&	 34	&	 Kien Tjin-Kam-Jet (UT), 	Distributed Deep Web Search\\
	&	 35	&	 Abdallah El Ali (UvA), Minimal Mobile Human Computer Interaction\\
	&	 36	&	 Than Lam Hoang (TUe), 	Pattern Mining in Data Streams\\
	&	 37	&	 Dirk B\"{o}rner (OUN), Ambient Learning Displays\\
	&	 38	&	 Eelco den Heijer (VU), 	Autonomous Evolutionary Art\\
	&	 39	&	 Joop de Jong (TUD), A Method for Enterprise Ontology based Design of Enterprise Information Systems\\
	&	 40	&	 Pim Nijssen (UM), Monte-Carlo Tree Search for Multi-Player Games\\
	&	 41	&	 Jochem Liem (UVA), Supporting the Conceptual Modelling of Dynamic Systems: A Knowledge Engineering Perspective on Qualitative Reasoning\\
	&	 42	&	 L\'{e}on Planken (TUD), Algorithms for Simple Temporal Reasoning\\
	&	 43	&	 Marc Bron (UVA), Exploration and Contextualization through Interaction and Concepts\\
	
\midrule
2014&	 01	&	 Nicola Barile (UU), Studies in Learning Monotone Models from Data\\
	&	 02	&	 Fiona Tuliyano (RUN), Combining System Dynamics with a Domain Modeling Method\\
	&	 03	&	 Sergio Raul Duarte Torres (UT), Information Retrieval for Children: Search Behavior and Solutions\\
	&	 04	&	 Hanna Jochmann-Mannak (UT), Websites for children: search strategies and interface design - Three studies on children's search performance and evaluation\\
	&	 05	&	 Jurriaan van Reijsen (UU), Knowledge Perspectives on Advancing Dynamic Capability\\
	&	 06	&	 Damian Tamburri (VU), Supporting Networked Software Development\\
	&	 07	&	 Arya Adriansyah (TUE), Aligning Observed and Modeled Behavior\\
	&	 08	&	 Samur Araujo (TUD), Data Integration over Distributed and Heterogeneous Data Endpoints\\
	&	 09	&	 Philip Jackson (UvT), Toward Human-Level Artificial Intelligence: Representation and Computation of Meaning in Natural Language\\
	&	 10	&	 Ivan Salvador Razo Zapata (VU), Service Value Networks\\
	&	 11	&	 Janneke van der Zwaan (TUD), An Empathic Virtual Buddy for Social Support\\
	&	 12	&	 Willem van Willigen (VU), Look Ma, No Hands: Aspects of Autonomous Vehicle Control\\
	&	 13	&	 Arlette van Wissen (VU), Agent-Based Support for Behavior Change: Models and Applications in Health and Safety Domains\\
	&	 14	&	 Yangyang Shi (TUD), Language Models With Meta-information\\
	&	 15	&	 Natalya Mogles (VU), Agent-Based Analysis and Support of Human Functioning in Complex Socio-Technical Systems: Applications in Safety and Healthcare\\
	&	 16	&	 Krystyna Milian (VU), Supporting trial recruitment and design by automatically interpreting eligibility criteria\\
	&	 17	&	 Kathrin Dentler (VU), Computing healthcare quality indicators automatically: Secondary Use of Patient Data and Semantic Interoperability\\
	&	 18	&	 Mattijs Ghijsen (UVA), Methods and Models for the Design and Study of Dynamic Agent Organizations\\
	&	 19	&	 Vinicius Ramos (TUE), 	Adaptive Hypermedia Courses: Qualitative and Quantitative Evaluation and Tool Support\\
	&	 20	&	 Mena Habib (UT), Named Entity Extraction and Disambiguation for Informal Text: The Missing Link\\
	&	 21	&	 Kassidy Clark (TUD), 	Negotiation and Monitoring in Open Environments\\
	&	 22	&	 Marieke Peeters (UU), Personalized Educational Games - Developing agent-supported scenario-based training\\
	&	 23	&	 Eleftherios Sidirourgos (UvA/CWI), 	Space Efficient Indexes for the Big Data Era\\
	&	 24	&	 Davide Ceolin (VU), Trusting Semi-structured Web Data\\
	&	 25	&	 Martijn Lappenschaar (RUN), 	New network models for the analysis of disease interaction\\
	&	 26	&	 Tim Baarslag (TUD), What to Bid and When to Stop\\
	&	 27	&	 Rui Jorge Almeida (EUR), 	Conditional Density Models Integrating Fuzzy and Probabilistic Representations of Uncertainty\\
	&	 28	&	 Anna Chmielowiec (VU), 	Decentralized k-Clique Matching\\
	&	 29	&	 Jaap Kabbedijk (UU), 	Variability in Multi-Tenant Enterprise Software\\
	&	 30	&	 Peter de Cock (UvT), 	Anticipating Criminal Behaviour\\
	&	 31	&	 Leo van Moergestel (UU), 	Agent Technology in Agile Multiparallel Manufacturing and Product Support\\
	&	 32	&	 Naser Ayat (UvA), 	On Entity Resolution in Probabilistic Data\\
	&	 33	&	 Tesfa Tegegne (RUN), Service Discovery in eHealth\\
	&	 34	&	 Christina Manteli (VU), The Effect of Governance in Global Software Development: Analyzing Transactive Memory Systems.\\
	&	 35	&	 Joost van Ooijen (UU), 	Cognitive Agents in Virtual Worlds: A Middleware Design Approach\\
	&	 36	&	 Joos Buijs (TUE), 	Flexible Evolutionary Algorithms for Mining Structured Process Models\\
	&	 37	&	 Maral Dadvar (UT), 	Experts and Machines United Against Cyberbullying\\
	&	 38	&	 Danny Plass-Oude Bos (UT), 	Making brain-computer interfaces better: improving usability through post-processing.\\
	&	 39	&	 Jasmina Maric (UvT), 	Web Communities, Immigration, and Social Capital\\
	&	 40	&	 Walter Omona (RUN), 	A Framework for Knowledge Management Using ICT in Higher Education\\
	&	 41	&	 Frederic Hogenboom (EUR), 	Automated Detection of Financial Events in News Text\\
	&	 42	&	 Carsten Eijckhof (CWI/TUD), 	Contextual Multidimensional Relevance Models\\
	&	 43	&	 Kevin Vlaanderen (UU), 	Supporting Process Improvement using Method Increments\\
	&	 44	&	 Paulien Meesters (UvT), 	Intelligent Blauw. Met als ondertitel: Intelligence-gestuurde politiezorg in gebiedsgebonden eenheden.\\
	&	 45	&	 Birgit Schmitz (OUN), 	Mobile Games for Learning: A Pattern-Based Approach\\
	&	 46	&	 Ke Tao (TUD), 	Social Web Data Analytics: Relevance, Redundancy, Diversity\\
	&	 47	&	 Shangsong Liang (UVA), 	Fusion and Diversification in Information Retrieval\\
	
\midrule
2015&	 01	&	 Niels Netten (UvA), Machine Learning for Relevance of Information in Crisis Response\\
	&	 02	&	 Faiza Bukhsh (UvT), Smart auditing: Innovative Compliance Checking in Customs Controls\\
	&	 03	&	 Twan van Laarhoven (RUN), Machine learning for network data\\
	&	 04	&	 Howard Spoelstra (OUN), Collaborations in Open Learning Environments\\
	&	 05	&	 Christoph B\"{o}sch (UT), Cryptographically Enforced Search Pattern Hiding\\
	&	 06	&	 Farideh Heidari (TUD), Business Process Quality Computation - Computing Non-Functional Requirements to Improve Business Processes\\
	&	 07	&	 Maria-Hendrike Peetz (UvA), Time-Aware Online Reputation Analysis\\
	&	 08	&	 Jie Jiang (TUD), 	Organizational Compliance: An agent-based model for designing and evaluating organizational interactions\\
	&	 09	&	 Randy Klaassen (UT), HCI Perspectives on Behavior Change Support Systems\\
	&	 10	&	 Henry Hermans (OUN), OpenU: design of an integrated system to support lifelong learning\\
	&	 11	&	 Yongming Luo (TUE), Designing algorithms for big graph datasets: A study of computing bisimulation and joins\\
	&	 12	&	 Julie M. Birkholz (VU), Modi Operandi of Social Network Dynamics: The Effect of Context on Scientific Collaboration Networks\\
	&	 13	&	 Giuseppe Procaccianti (VU), Energy-Efficient Software\\
	&	 14	&	 Bart van Straalen (UT), A cognitive approach to modeling bad news conversations\\
	&	 15	&	 Klaas Andries de Graaf (VU), Ontology-based Software Architecture Documentation\\
	&	 16	&	 Changyun Wei (UT), Cognitive Coordination for Cooperative Multi-Robot Teamwork\\
	&	 17	&	 Andr\'{e} van Cleeff (UT), Physical and Digital Security Mechanisms: Properties, Combinations and Trade-offs\\
	&	 18	&	 Holger Pirk (CWI), Waste Not, Want Not! - Managing Relational Data in Asymmetric Memories\\
	&	 19	&	 Bernardo Tabuenca (OUN), Ubiquitous Technology for Lifelong Learners\\
	&	 20	&	 Lois Vanh\'{e}e (UU), 	Using Culture and Values to Support Flexible Coordination\\
	&	 21	&	 Sibren Fetter (OUN), Using Peer-Support to Expand and Stabilize Online Learning\\
	&	 22	&	 Zhemin Zhu (UT), 	Co-occurrence Rate Networks\\
	&	 23	&	 Luit Gazendam (VU), Cataloguer Support in Cultural Heritage\\
	&	 24	&	 Richard Berendsen (UVA), 	Finding People, Papers, and Posts: Vertical Search Algorithms and Evaluation\\
	&	 25	&	 Steven Woudenberg (UU), Bayesian Tools for Early Disease Detection\\
	&	 26	&	 Alexander Hogenboom (EUR), Sentiment Analysis of Text Guided by Semantics and Structure\\
	&	 27	&	 S\'{a}ndor H\'{e}man (CWI), Updating compressed colomn stores\\
	&	 28	&	 Janet Bagorogoza (TiU), Knowledge Management and High Performance; The Uganda Financial Institutions Model for HPO\\
	&	 29	&	 Hendrik Baier (UM), Monte-Carlo Tree Search Enhancements for One-Player and Two-Player Domains\\
	&	 30	&	 Kiavash Bahreini (OU), Real-time Multimodal Emotion Recognition in E-Learning\\
	&	 31	&	 Yakup Ko\c{c} (TUD), On the robustness of Power Grids\\
	&	 32	&	 Jerome Gard (UL), Corporate Venture Management in SMEs\\
	&	 33	&	 Frederik Schadd (TUD), Ontology Mapping with Auxiliary Resources\\
	&	 34	&	 Victor de Graaf (UT), Gesocial Recommender Systems\\
	&	 35	&	 Jungxao Xu (TUD), Affective Body Language of Humanoid Robots: Perception and Effects in Human Robot Interaction\\

\midrule
2016&	 01	&	 Syed Saiden Abbas (RUN), Recognition of Shapes by Humans and Machines\\
	&	 02	&	 Michiel Christiaan Meulendijk (UU), Optimizing medication reviews through decision support: prescribing a better pill to swallow\\
	&	 03	&	 Maya Sappelli (RUN), Knowledge Work in Context: User Centered Knowledge Worker Support\\
	&	 04	&	 Laurens Rietveld (VU), Publishing and Consuming Linked Data\\
	&	 05	&	 Evgeny Sherkhonov (UVA), Expanded Acyclic Queries: Containment and an Application in Explaining Missing Answers\\
	&	 06	&	 Michel Wilson (TUD), Robust scheduling in an uncertain environment\\
	&	 07	&	 Jeroen de Man (VU), Measuring and modeling negative emotions for virtual training\\
	&	 08	&	 Matje van de Camp (TiU), A Link to the Past: Constructing Historical Social Networks from Unstructured Data\\
	&	 09	&	 Archana Nottamkandath (VU), Trusting Crowdsourced Information on Cultural Artefacts\\
	&	 10	&	 George Karafotias (VUA), Parameter Control for Evolutionary Algorithms\\
	&	 11	&	 Anne Schuth (UVA), Search Engines that Learn from Their Users\\
	&	 12	&	 Max Knobbout (UU), Logics for Modelling and Verifying Normative Multi-Agent Systems\\
	&	 13	&	 Nana Baah Gyan (VU), The Web, Speech Technologies and Rural Development in West Africa - An ICT4D Approach\\
	&	 14	&	 Ravi Khadka (UU), Revisiting Legacy Software System Modernization\\
	&	 15	&	 Steffen Michels (RUN), Hybrid Probabilistic Logics - Theoretical Aspects, Algorithms and Experiments\\
	&	 16	&	 Guangliang Li (UVA), Socially Intelligent Autonomous Agents that Learn from Human Reward\\
	&	 17	&	 Berend Weel (VU), Towards Embodied Evolution of Robot Organisms\\
	&	 18	&	 Albert Mero\~{n}o Pe\~{n}uela (VU), Refining Statistical Data on the Web\\
	&	 19	&	 Julia Efremova (Tu/e), Mining Social Structures from Genealogical Data\\
	&	 20	&	 Daan Odijk (UVA), Context \& Semantics in News \& Web Search\\
	&	 21	&	 Alejandro Moreno C\'{e}lleri (UT), From Traditional to Interactive Playspaces: Automatic Analysis of Player Behavior in the Interactive Tag Playground\\
	&	 22	&	 Grace Lewis (VU), Software Architecture Strategies for Cyber-Foraging Systems\\
	&	 23	&	 Fei Cai (UVA), Query Auto Completion in Information Retrieval\\
	&	 24	&	 Brend Wanders (UT), Repurposing and Probabilistic Integration of Data; An Iterative and data model independent approach\\
	&	 25	&	 Julia Kiseleva (TU/e), Using Contextual Information to Understand Searching and Browsing Behavior\\
	&	 26	&	 Dilhan Thilakarathne (VU), In or Out of Control: Exploring Computational Models to Study the Role of Human Awareness and Control in Behavioural Choices, with Applications in Aviation and Energy Management Domains\\
	&	 27	&	 Wen Li (TUD), Understanding Geo-spatial Information on Social Media\\
	&	 28	&	 Mingxin Zhang (TUD), Large-scale Agent-based Social Simulation - A study on epidemic prediction and control\\
	&	 29	&	 Nicolas H\"{o}ning (TUD), Peak reduction in decentralised electricity systems - Markets and prices for flexible planning\\
	&	 30	&	 Ruud Mattheij (UvT), The Eyes Have It\\
	&	 31	&	 Mohammad Khelghati (UT), Deep web content monitoring\\
	&	 32	&	 Eelco Vriezekolk (UT), Assessing Telecommunication Service Availability Risks for Crisis Organisations\\
	&	 33	&	 Peter Bloem (UVA), Single Sample Statistics, exercises in learning from just one example\\
	&	 34	&	 Dennis Schunselaar (TUE), Configurable Process Trees: Elicitation, Analysis, and Enactment\\
	&	 35	&	 Zhaochun Ren (UVA), Monitoring Social Media: Summarization, Classification and Recommendation\\
	&	 36	&	 Daphne Karreman (UT), Beyond R2D2: The design of nonverbal interaction behavior optimized for robot-specific morphologies\\
	&	 37	&	 Giovanni Sileno (UvA), Aligning Law and Action - a conceptual and computational inquiry\\
	&	 38	&	 Andrea Minuto (UT), Materials that Matter - Smart Materials meet Art \& Interaction Design\\
	&	 39	&	 Merijn Bruijnes (UT), Believable Suspect Agents; Response and Interpersonal Style Selection for an Artificial Suspect\\
	&	 40	&	 Christian Detweiler (TUD), Accounting for Values in Design\\
	&	 41	&	 Thomas King (TUD), Governing Governance: A Formal Framework for Analysing Institutional Design and Enactment Governance\\
	&	 42	&	 Spyros Martzoukos (UVA), Combinatorial and Compositional Aspects of Bilingual Aligned Corpora\\
	&	 43	&	 Saskia Koldijk (RUN), Context-Aware Support for Stress Self-Management: From Theory to Practice\\
	&	 44 &	 Thibault Sellam (UVA), Automatic Assistants for Database Exploration\\
	&	 45	&	 Bram van de Laar (UT), Experiencing Brain-Computer Interface Control\\
	&	 46	&	 Jorge Gallego Perez (UT), Robots to Make you Happy\\
	&	 47	&	 Christina Weber (UL), Real-time foresight - Preparedness for dynamic innovation networks\\
	&	 48	&	 Tanja Buttler (TUD), Collecting Lessons Learned\\
	&	 49	&	 Gleb Polevoy (TUD), Participation and Interaction in Projects. A Game-Theoretic Analysis\\
	&	 50	&	 Yan Wang (UVT), The Bridge of Dreams: Towards a Method for Operational Performance Alignment in IT-enabled Service Supply Chains\\
	
\midrule
2017&	 01	&	 Jan-Jaap Oerlemans (UL), Investigating Cybercrime\\
	&	 02	&	 Sjoerd Timmer (UU), Designing and Understanding Forensic Bayesian Networks using Argumentation\\
	&	 03	&	 Dani\"{e}l Harold Telgen (UU), Grid Manufacturing; A Cyber-Physical Approach with Autonomous Products and Reconfigurable Manufacturing Machines\\
	&	 04	&	 Mrunal Gawade (CWI), Multi-core Parallelism in a Column-store\\
	&	 05	&	 Mahdieh Shadi (UVA), Collaboration Behavior\\
	&	 06	&	 Damir Vandic (EUR), Intelligent Information Systems for Web Product Search\\
	&	 07	&	 Roel Bertens (UU), Insight in Information: from Abstract to Anomaly\\
	&	 08	& 	 Rob Konijn (VU)	, Detecting Interesting Differences:Data Mining in Health Insurance Data using Outlier Detection and Subgroup Discovery\\
	&	 09	&	 Dong Nguyen (UT), Text as Social and Cultural Data: A Computational Perspective on Variation in Text\\
	&	 10	&	 Robby van Delden (UT), (Steering) Interactive Play Behavior\\       
	&	 11	&	 Florian Kunneman (RUN), Modelling patterns of time and emotion in Twitter \#anticipointment\\	      										
	&	 12	&	 Sander Leemans (TUE), Robust Process Mining with Guarantees\\      
 	&	 13	& 	 Gijs Huisman (UT), Social Touch Technology - Extending the reach of social touch through haptic technology\\     
 	&	 14	&	 Shoshannah Tekofsky (UvT), You Are Who You Play You Are: Modelling Player Traits from Video Game Behavior\\ 
	&	 15	&	 Peter Berck (RUN), Memory-Based Text Correction\\  
	&	 16	&	 Aleksandr Chuklin (UVA), Understanding and Modeling Users of Modern Search Engines\\   
	&	 17	&	 Daniel Dimov (UL), Crowdsourced Online Dispute Resolution\\
	&	 18	&	 Ridho Reinanda (UVA), Entity Associations for Search\\
	&	 19	& 	 Jeroen Vuurens (UT), Proximity of Terms, Texts and Semantic Vectors in Information Retrieval\\
	&	 20	&	 Mohammadbashir Sedighi (TUD), Fostering Engagement in Knowledge Sharing: The Role of Perceived Benefits, Costs and Visibility\\
	&	 21	&	 Jeroen Linssen (UT), Meta Matters in Interactive Storytelling and Serious Gaming (A Play on Worlds)\\
	&	 22	&	 Sara Magliacane (VU), Logics for causal inference under uncertainty\\
	&	 23	&	 David Graus (UVA), Entities of Interest --- Discovery in Digital Traces\\
	&	 24	&	 Chang Wang (TUD), Use of Affordances for Efficient Robot Learning\\
	&	 25	&	 Veruska Zamborlini (VU), Knowledge Representation for Clinical Guidelines, with applications to Multimorbidity Analysis and Literature Search\\
	&	 26	&	 Merel Jung (UT), Socially intelligent robots that understand and respond to human touch\\	
	&	 27	&	 Michiel Joosse (UT), Investigating Positioning and Gaze Behaviors of Social Robots: People's Preferences, Perceptions and Behaviors\\
	&	 28	&	 John Klein (VU), Architecture Practices for Complex Contexts\\
	&	 29	&	 Adel Alhuraibi (UvT), From IT-BusinessStrategic Alignment to Performance: A Moderated Mediation Model of Social Innovation, and Enterprise Governance of    IT"\\
	&	 30	&	 Wilma Latuny (UvT), The Power of Facial Expressions\\
	&	 31	&	 Ben Ruijl (UL), Advances in computational methods for QFT calculations\\
	&	 32	& 	 Thaer Samar (RUN), Access to and Retrievability of Content in Web Archives\\
	&	 33	&	 Brigit van Loggem (OU), Towards a Design Rationale for Software Documentation: A Model of Computer-Mediated Activity\\
	&	 34	&	 Maren Scheffel (OU), The Evaluation Framework for Learning Analytics \\
	&	 35	&	 Martine de Vos (VU), Interpreting natural science spreadsheets \\
	&	 36	&	 Yuanhao Guo (UL), Shape Analysis for Phenotype Characterisation from High-throughput Imaging \\
	&	 37	&	 Alejandro Montes Garcia (TUE), WiBAF: A Within Browser Adaptation Framework that Enables Control over Privacy \\
	&	 38	&	 Alex Kayal (TUD), Normative Social Applications \\	 
	&	 39	&	 Sara Ahmadi (RUN), Exploiting properties of the human auditory system and compressive sensing methods to increase   noise robustness in ASR \\
	&	 40	&	 Altaf Hussain Abro (VUA), Steer your Mind: Computational Exploration of Human Control in Relation to Emotions, Desires and Social Support For applications in human-aware support systems \\
	&	 41	&	 Adnan Manzoor (VUA), Minding a Healthy Lifestyle: An Exploration of Mental Processes and a Smart Environment to Provide Support for a Healthy Lifestyle\\
	&	 42	&	 Elena Sokolova (RUN), Causal discovery from mixed and missing data with applications on ADHD  datasets\\
	&	 43	&	 Maaike de Boer (RUN), Semantic Mapping in Video Retrieval\\
	&	 44	&	 Garm Lucassen (UU), Understanding User Stories - Computational Linguistics in Agile Requirements Engineering\\
	&	 45	&	 Bas Testerink	(UU), Decentralized Runtime Norm Enforcement\\
	&	 46	&	 Jan Schneider	(OU), Sensor-based Learning Support\\
	&	 47	&	 Jie Yang (TUD), Crowd Knowledge Creation Acceleration\\
	&	 48	&	 Angel Suarez (OU), Collaborative inquiry-based learning\\
	
\midrule
2018&	 01	&	 Han van der Aa (VUA), Comparing and Aligning Process Representations \\ 
	&	 02	&	 Felix Mannhardt (TUE), Multi-perspective Process Mining \\
	&	 03	&	 Steven Bosems (UT), Causal Models For Well-Being: Knowledge Modeling, Model-Driven Development of Context-Aware Applications, and Behavior Prediction\\
	&	 04	&	 Jordan Janeiro (TUD), Flexible Coordination Support for Diagnosis Teams in Data-Centric Engineering Tasks \\
	&	 05	&	 Hugo Huurdeman (UVA), Supporting the Complex Dynamics of the Information Seeking Process \\
	&	 06	&	 Dan Ionita (UT), Model-Driven Information Security Risk Assessment of Socio-Technical Systems \\
	&	 07	&	 Jieting Luo (UU), A formal account of opportunism in multi-agent systems \\
	&	 08	&	 Rick Smetsers (RUN), Advances in Model Learning for Software Systems \\
	&	 09	&	 Xu Xie	(TUD), Data Assimilation in Discrete Event Simulations \\	
	&	 10	&	 Julienka Mollee (VUA), Moving forward: supporting physical activity behavior change through intelligent technology \\
	&	 11	&	 Mahdi Sargolzaei (UVA), Enabling Framework for Service-oriented Collaborative Networks \\
	&	 12	&	 Xixi Lu (TUE), Using behavioral context in process mining \\
	&	 13	&	 Seyed Amin Tabatabaei (VUA), Computing a Sustainable Future \\
	&	 14	&	 Bart Joosten (UVT), Detecting Social Signals with Spatiotemporal Gabor Filters \\
	&	 15	&	 Naser Davarzani (UM), Biomarker discovery in heart failure \\
	&	 16	&	 Jaebok Kim (UT), Automatic recognition of engagement and emotion in a group of children \\
	&	 17	&	 Jianpeng Zhang (TUE), On Graph Sample Clustering \\
	&	 18	& 	 Henriette Nakad (UL), De Notaris en Private Rechtspraak \\
	&	 19	&	 Minh Duc Pham (VUA), Emergent relational schemas for RDF \\
	&	 20	&	 Manxia Liu (RUN), Time and Bayesian Networks \\
	&	 21	&	 Aad Slootmaker (OUN), EMERGO: a generic platform for authoring and playing scenario-based serious games \\
	&	 22	&	 Eric Fernandes de Mello Araujo (VUA), Contagious: Modeling the Spread of Behaviours, Perceptions and Emotions in Social Networks \\
	&	 23	&	 Kim Schouten (EUR), Semantics-driven Aspect-Based Sentiment Analysis \\
	&	 24	&	 Jered Vroon (UT), Responsive Social Positioning Behaviour for Semi-Autonomous Telepresence Robots \\
	&	 25	&	 Riste Gligorov (VUA), Serious Games in Audio-Visual Collections \\ 
	&	 26	& 	 Roelof Anne Jelle de Vries (UT),Theory-Based and Tailor-Made: Motivational Messages for Behavior Change Technology \\ 
	&	 27	&	 Maikel Leemans (TUE), Hierarchical Process Mining for Scalable Software Analysis \\
	&	 28	&	 Christian Willemse (UT), Social Touch Technologies: How they feel and how they make you feel \\	
	&	 29	&	 Yu Gu (UVT), Emotion Recognition from Mandarin Speech \\
	&	 30	&	 Wouter Beek,  The "K" in "semantic web" stands for "knowledge": scaling semantics to the web \\
	
\midrule
2019&	 01	&	 Rob van Eijk (UL),Comparing and Aligning Process Representations \\
 	&	 02	&	 Emmanuelle Beauxis Aussalet (CWI, UU), Statistics and Visualizations for Assessing Class Size Uncertainty \\
 	&	 03	&	 Eduardo Gonzalez Lopez de Murillas (TUE), Process Mining on Databases: Extracting Event Data from Real Life Data Sources \\
 	&	 04	&	 Ridho Rahmadi (RUN), Finding stable causal structures from clinical data \\				 
 	& 	 05	&	 Sebastiaan van Zelst (TUE), Process Mining with Streaming Data \\
 	&	 06	& 	 Chris Dijkshoorn (VU), Nichesourcing for Improving Access to Linked Cultural Heritage Datasets \\
 	&	 07	&	 Soude Fazeli (TUD), \\
 	& 	 08	&	 Frits de Nijs (TUD), Resource-constrained Multi-agent Markov Decision Processes \\
 	&	 09	&	 Fahimeh Alizadeh Moghaddam (UVA), Self-adaptation for energy efficiency in software systems \\
 	&	 10	&	 Qing Chuan Ye (EUR), Multi-objective Optimization Methods for Allocation and Prediction \\
 	&	 11	&	 Yue Zhao (TUD), Learning Analytics Technology to Understand Learner Behavioral Engagement in MOOCs \\
 	&	 12	&	 Jacqueline Heinerman (VU), Better Together \\
 	&	 13	&	 Guanliang Chen (TUD), MOOC Analytics: Learner Modeling and Content Generation \\
 	&	 14	&	Daniel Davis (TUD), Large-Scale Learning Analytics: Modeling Learner Behavior \& Improving Learning Outcomes in Massive Open Online Courses \\
 	&	 15	&	 Erwin Walraven (TUD), Planning under Uncertainty in Constrained and Partially \\
 	&	 16	&	 Guangming Li (TUE), Process Mining based on Object-Centric Behavioral Constraint (OCBC) Models \\
 	&	 17	&	 Ali (RUN) H\"{u}rriyeto\v{g}lu, Extracting Actionable Information from Microtexts \\
\bottomrule
%\end{longtable}
\end{longtabu}
